A Multiwavelength Spectral and Polarimetric Study of the Jet of 3C 264

We present a comprehensive multiband spectral and polarimetric study of the jet of 3C 264 (NGC 3862). Included in this study are three HST optical and ultraviolet polarimetry data sets, along with new and archival VLA radio imaging and polarimetry, a re-analysis of numerous HST broadband data sets from the near infrared to the far ultraviolet, and a Chandra ACIS-S observation. We investigate similarities and differences between optical and radio polarimetry, in both degree of polarization and projected magnetic field direction. We also examine the broadband spectral energy distribution of both the nucleus and jet of 3C 264, from the radio through the X-rays. From this we place constraints on the physics of the 3C 264 system, the jet and its dynamics. We find significant curvature of the spectrum from the near-IR to ultraviolet, and synchrotron breaks steeper than 0.5, a situation also encountered in the jet of M87. This likely indicates velocity and/or magnetic field gradients and more efficient particle acceleration localized in the faster/higher magnetic field parts of the flow. The magnetic field structure of the 3C 264 jet is remarkably smooth; however, we do find complex magnetic field structure that is correlated with changes in the optical spectrum. We find that the X-ray emission is due to the synchrotron process; we model the jet spectrum and discuss mechanisms for accelerating particles to the needed energies, together with implications for the orientation of the jet under a possible spine-sheath model.

==> bibliography.tex <==
\begin{thebibliography}{}

\bibitem[Aloy et al. 2003]{Aloy03} Aloy, M.-A., Marti, J. M., Gomez, J. L.,
Agudo, I., Ibanez, J. M., 2003, ApJ, 585, L109  

\bibitem[Anderson \& King 2003]{Anderson03} Anderson, J., King, I., 2003, 
PASP, 803, 113, 2003

\bibitem[Anderson \& King 2004]{Anderson04} Anderson, J., ,King, I., 2004, 
ACS Instrument Science Report, ACS 04-15

\bibitem[Baum et al. 2006]{Baum06} Baum, S., Franz, G., Kastner, J., Perlman,
E., O'Dea, C., 2006, AAS Meeting 207, \#79.04

\bibitem[Baum et al. 1992]{Baum92} Baum, S. A., Heckman, T. M., van Breugel,
W., 1992, ApJ, 389, 208

\bibitem[Baum et al. 1990]{Baum90} Baum, S. A., Heckman, T., van Breugel, W., 
1990, ApJS, 74, 389
 
\bibitem[Baum et al 1997]{Baum97} Baum, S. et al,
ApJ, 483, 178, 1997

\bibitem[Baum et al. 1998]{Baum98} Baum, S., et al., 1998, ApJ, 492, 854

%\bibitem[Bell 1997]{Bell} Bell, J., {\it Vistas in Astronomy}, 41, 87, 1997.

%\bibitem[Biretta et al 2004]{Biretta04} Biretta, J., V. Kozhurina-Platais, F.
%Boffi, W. Sparks, and J. Walsh, ACS Instrument Science Report, ISR 04-09, 2004.

\bibitem[Biretta et al, 1999]{Biretta99} Biretta, J.A.,  Sparks, W. B., 
Macchetto, F., 1999, ApJ, 520, 621

\bibitem[Biretta et al. 1995]{Biretta95} Biretta, J. A., Zhou, F., Owen, F. N.,
1995, ApJ, 447, 582

%\bibitem[Biretta \& McMaster 1997]{Biretta97} Biretta, J.A., and McMaster, M.,
%1997, WFPC2 Instrument Science Report, ISR 97-11

%\bibitem[Birk \& Lesch 2000]{BL00} Birk, G. T., Lesch, H., 2000, ApJ, 530, L77 

\bibitem[Bliss et al.(2009)]{bliss} 
Bliss, A.F., Worrall, D.M., Birkinshaw, M., Murray, S.S., Tananbaum
H., 2009, ApJ, 698, 1061

\bibitem[Bridle 1996]{Bridle96} Bridle, A. H., 1996, in Energy Transport in Radio
Galaxies and Quasars, ed. Hardee, P. E., Bridle, A. H., \& Zensus, J. A. (San
Francisco: PASP), p. 383  

\bibitem[Bridle \& Vallee 1981]{bv81} Bridle, A. H., Vallee, J. P., 1981, AJ,
86, 1165

\bibitem[Carter et al. 2003]{Carter03} Carter, C., Karovska, M., Jerius, D.,
Glotfelty, K., Beikman, S., 2003, Astrophysical Data Analysis Software and 
Systems XII, ASP Conference Series, v. 295, 477 

\bibitem[Chiaberge et al. 1999]{Chiaberge99} Chiaberge, M., Capetti, A.,
Celotti, A., 1999, A \& A, 349, 77

\bibitem[Cheung et al. 2007]{cheung07} Cheung, C. C., Harris, D. E., Stawarz,
L., 2007, ApJL, 663, L5

\bibitem[Civano et al.(2007)]{civano} 
Civano, F.~et al., 2007, A\&A, 476, 1223

\bibitem[Colgate \& Li 1999]{Colgate99} Colgate, S. A., Li, H., Proceedings
of IAU Symposium \#195, (San Francisco: Astronomical Society of the Pacific),
255, 1999.

\bibitem[Cotton et al. 1995]{Cotton95} Cotton, W. D., Feretti, L., Giovannini,
G., Venturi, T., Lara, L., Marcaide, J., Wehrle, A. E., 1995, ApJ, 452, 605 

\bibitem[Cortese et al. 2004]{Cortese04} Cortese, L., Gavazzi, G., Boselli,
A., Iglesias-Paramo, J., Carrasco, L., 2004, A\& A, 
425, 429 

\bibitem[Crane et al. 1993]{Crane93} Crane, P., et al, 1993, ApJ,
402, L37

\bibitem[Curtis 1918]{Curtis18} Curtis, H. D., 1918 {\it Publications of Lick
Observatory}, 13, 9

\bibitem[De Young 2002]{DeYoung} De Young, D. S., 2002, The Physics of
Extragalactic Radio Sources, (Chicago, Ill.: University of Chicago Press)

\bibitem[Dickenson et al. 2004]{Dickenson04} Dickenson, M., B. Mobasher and E.
Roye, ed., 2004, HST Data Handbook for NICMOS, Version 6.0 (Baltimore: STScI)

\bibitem[Dickey \& Lockman 1990]{dlock90} Dickey,
  J. M. \& Lockman, F. J., 1990, ARA\&A, 28, 215

\bibitem[Donato et al. 2004]{Donato04} Donato, D., Sambruna, R. M., Gliozzi, 
M., 2004, ApJ, 617, 915

\bibitem[Dulwich et al. 2007]{Dulwich07} Dulwich, F., Worrall, D. M., 
Birkinshaw, M., Padgett, C. A., Perlman, E. S., 2007, MNRAS, 374, 1216

\bibitem[Dulwich et al. 2009]{Dulwich09} Dulwich, F., Worrall, D. M., 
Birkinshaw, M., Padgett, C. A., Perlman, E. S., 2009, MNRAS, in press

\bibitem[Dunkley et al. 2009]{Dunkley09} Dunkley, J., et al., 2009, ApJS, 180,
306 

\bibitem[Edge et al. 1959]{Edge59} Edge, D. O., Shakeshaft, J. R., McAdam, W.
B., Baldwin, J. E., Archer, S., 1959, Mem. R. Astron. Soc., 68, 37

\bibitem[Elvis et al. 1981]{Elvis81} Elvis, M., Schreier, E. J., Tonry, J., 
Davis, M., Huchra, J. P., 1981, ApJ, 246, 20

\bibitem[Evans et al. 2006]{Evans06} Evans, D. A., Worrall, D. M., Hardcastle,
M. J., Kraft, R. P., Birkinshaw, M., 2006, ApJ, 642, 96

\bibitem[Fanaroff \& Riley 1974]{FR} Fanaroff, B. L., Riley, J. M., 
1974, MNRAS 167, 31 

\bibitem[Fasano et al. 1996]{Fasano96} Fasano, G., R. Falomo, and R. Scarpa,
1996, MNRAS, 282, 40

\bibitem[Fender 2001]{Fender} Fender, R.P., 2001, AIP Conference Proceedings, ed.
N.E. White, G. Malaguti, and G. Pamumbo, 599, 101

\bibitem[Fleishman 2006]{fl06} Fleishman, G. D., 2006, MNRAS, 365, L11

\bibitem[Floyd et al. 2006]{floyd06} Floyd, D. J. E., 
% Perlman, E., Leahy, J. 
% P., Beswick, R. J., Jackson, N. J., Sparks, W. B., Axon, D. J., O'Dea, C. P., 
et al., 2006, ApJ, 639, 23

\bibitem[Ford et al. 1994]{ford94} Ford, H.C., et al., 1994, ApJL, 435, L27
 
\bibitem[Georganopoulos \& Kazanas 2003]{Georg03} 
Georganopoulos, M., Kazanas, D., 2003, ApJ, 594, L27

\bibitem[Ghisellini et al. 2005]{Ghisellini05} Ghisellini, G., Tavecchio, F.,
Chiaberge, M., 2005, A\& A, 432, 401

\bibitem[Gonz\`alez-Delgado \& P\'erez 1993]{Gonzalez93} Gonz\`alez-Delgado,
R. M., P\'erez, E., ApSS, 205, 127, 1993.

\bibitem[Govoni et al. 2000]{Govoni00} Govoni, F., Falomo, R., Fasano, G.,
Scarpa, R., A\& A, 353, 507, 2000.

\bibitem[Hardcastle et al. 2007]{hard07} Hardcastle, M. J., et al., 2007, 
ApJ, 670, L81

\bibitem[Hardcastle et al. 2006]{hard06} Hardcastle, M. J., Kraft, R. P.,
Worrall, D. M., 2006, MNRAS, 368, L15

\bibitem[Hardcastle et al. 2003]{hard03} Hardcastle, M. J., Worrall, D. M., 
Kraft, R. P., Forman, W. R., 
Jones, C., Murray, S. S., 2003, ApJ, 593, 169
   
\bibitem[Heyer et al. 2004]{Heyer04} Heyer, I., WFPC2
Instrument Handbook, Version 9.0 (Baltimore: STScI), 2004.

\bibitem[{\it Beams and Jets in Astrophysics}, 1991]{Hughes91} Hughes, P. A.,
1991, Beams and Jets
in Astrophysics, (Cambridge: Cambridge University Press)

\bibitem[Hutchings et al.(1998)]{hutchings} 
Hutchings, J.B., Baum, S.A., Weistrop, D., Nelson, C., Kaiser, M.E.,
Gelderman, R.F., 1998, AJ, 116, 634

\bibitem[Jaffe \& Perola 1973]{Jaffe73} Jaffe, W. J., Perola, G. C., A \& A, 
26, 421, 1973.

\bibitem[Jester et al. 2006]{Jester06} Jester, S., Harris, D. E., Marshall, H.
L., Meisenheimer, K., 2006, ApJ, 648, 900

\bibitem[Jester et al. 2005]{Jester05} Jester, S., R\"oser, H.--J., 
Meisenheimer, K., Perley, R., 2005, A\& A, 431, 477

\bibitem[Jester et al. 2001]{Jester01} Jester, S., R\"oser, H.--J.,
Meisenheimer, K., Perley, R., Conway, R., 2001, A\& A, 373, 447  

\bibitem[Kardashev 1962]{Kardashev62} Kardashev, N. S., {\it Soviet
Astronomy}, 6, 317, 1962.

\bibitem[Kharb et al. 2009]{Kharb09}
Kharb, P., Gabuzda, D. C., O'Dea, C. P., Shastri, P., Baum, S. A., 2009, ApJ, 
694, 1485

%\bibitem[Kollgaard 1994]{Kollgaard94} Kollgaard, R.I., {\it Vistas in
%Astronomy}, 1994, 38, 29

\bibitem[Laing 1996]{Laing96} Laing, R. A., 1996, in Energy Transport in Radio
Galaxies and Quasars, ed. Hardee, P. E., Bridle, A. H., \& Zensus, J. A. (San
Francisco: PASP), p. 241  

\bibitem[Laing et al. 2008]{Laing08}  Laing, R. A., Bridle, A. H., Parma, P., 
Feretti, L., Giovannini, G., Murgia, M., Perley, R. A., 2008, MNRAS, 386, 657

\bibitem[Lara et al. 1997]{Lara97} Lara, L.,  Cotton, W. D., Feretti, D., 
Giovannini, G., Venturi, T., Marcaide, J. M., 1997, ApJ, 
474, 179

\bibitem[Lara et al. 2004]{Lara04} Lara, L., Giovannini, G., Cotton, W. D.,
Feretti, L., Venturi, T., A \& A, 415, 905, 2004.

%\bibitem[Lawrence 1991]{Lawrence91} Lawrence, A., MNRAS, 252, 586, 1991.

\bibitem[Leahy et al. 1997]{Leahy97} Leahy, J. P.,
%Black,  A.R.S.,
%Dennett-Thorpe, J., Hardcastle, M.J.,Komissarov, S., Perley, R. A., Riley, J.M.,
%Scheuer, P.A.G., 
et al., 1997, MNRAS, 291, 20

%\bibitem[Lesch \& Birk 1998]{Lesch98} Lesch, H., Birk, G. T., ApJ,
%499, 167, 1998.

\bibitem[Li et al. 2004]{LI} Li, J.-Q., Kastner, J.H., Prigozhin,  G. Y.,
Schulz, N. S., Feigelson, E. D., Getman,  K. V., 2004, ApJ, 610,
1204.

\bibitem[Lipovka et al. 2005]{lipov} Lipovka, A. A., Lipovka, N. M.,
Gosachinskii, I. V., Chavira, E., 2005, Astron. Zh., 82, 483

\bibitem[Liu \& Shen 2007]{Liu} Liu, W.--P., Shen, Z.--Q., 2007, ApJ, 668, L23

\bibitem[Marshall et al. 2005]{Marshall05} Marshall, H. L., et al., 2005, 
ApJS, 156, 13

\bibitem[Martel et al. 1998]{Martel98} Martel, A. R., et al.,  1998, 
ApJ, 496, 203

\bibitem[Martel et al. 2000]{Martel00} Martel, A. R., Turner, N. J., Sparks, 
W. B., Baum, S. A., 2000, ApJS, 130, 267

\bibitem[Noel-Storr et al. 2003]{ns03} Noel-Storr, J., Baum, S. A., Verdoes
Kleijn, G., van der Marel, R. P., O'Dea, C. P., de Zeeuw, P. T., Carollo, C. M.,
2003, APJS, 148, 419 

\bibitem[Pacholczyk 1970]{Pacholczyk70} Pacholczyk, A.G., Radio Astrophysics,
(San Fransisco: Freeman), 1970

\bibitem[Pavlovsky 2005]{Pavlovsky05} Pavlovsky, C., et al, 2005, ACS Data
Handbook, Version 4.0 (Baltimore: STScI)

\bibitem[Perlman et al. 2006]{Perlman06} Perlman, E.S., et al,
2006, ApJ, 651, 735

\bibitem[Perlman \& Wilson 2005]{PW05} Perlman, E.S., and Wilson, A. S., 2005,
ApJ, 627, 140,

\bibitem[Perlman et al 2001]{Perlman01} Perlman, E.S., Biretta, J. A., 
Sparks, W. B., Macchetto, F. D., \& Leahy, J. P., 2001, ApJ, 551, 206

\bibitem[Perlman et al. 1999]{Perlman99} Perlman, E. S., Biretta, J. A., Zhou,
F., Sparks, W. B., \& Macchetto, F. D., 1999, AJ, 117, 2185, 
1999.

\bibitem[Reynolds 2009]{Reynolds09} Reyolds, S. P., 2009, ApJ, in press, 
arXiv:0907.4756

\bibitem[Sahayanathan 2008]{Saha08} Sahayanathan, S., 2008, MNRAS, 388, L49

\bibitem[Serkowski 1962]{Serkowski62} Serkowski, K., 1962, 
Advances in Astronomy
and Astrophysics, Academic Press 1, 289

\bibitem[Sun et al. 2007]{sun07} Sun, M., Jones, C., Forman, W.,
Vikhlinin, A., Donahue, M., Voit, M.,
2007, ApJ, 657, 197

\bibitem[Sun et al. 2005]{sun05} Sun, M., Vikhlinin, A., Forman, W., Jones, 
C., Murray, S. S., 2005, ApJ, 619, 169 

\bibitem[Tananbaum et al.(1997)]{tananbaum} Tananbaum, H., Tucker, W.,
Prestwich, A., Remillard, R., 1997, ApJ, 476, 83

\bibitem[Thomson et al. 1993]{thomson93} Thomson, R. C., Mackay, C. D., 
Wright, A. E., 1993, Nature, 365, 133

\bibitem[Tonry 1991]{Tonry91} Tonry, J. L., 1991, ApJ, 373, L1

\bibitem[Wang et al. 2009]{Wang09} Wang, Y., Kaiser, C. R., Laing, R. A., 
Alexander, P., Pavlovski, G., Knigge, C., 2009, MNRAS, 397, 1113

\bibitem[Worrall (2009)]{wreview} Worrall, D.M., 2009, A\&ARev, 17, 1

\bibitem[Worrall \& Birkinshaw(2006)]{wbreview} Worrall, D.M.,
Birkinshaw, M., 2006, Lect Notes Phys, 693, 39

\bibitem[Worrall et al.(1999)]{worrall} Worrall, D.M., Birkinshaw, M.,
Remillard, R.A., Prestwich, A., Tucker, W.H., Tananbaum, H., 1999, ApJ,
516, 163


\bibitem[Worrall \& Birkinshaw 2005]{wb05} Worrall, D. M., Birkinshaw, M.,
2005, MNRAS, 360, 926

\bibitem[Worrall et al. 2007]{Worr07} Worrall, D. M., Birkinshaw, M., Laing,
R. A., Cotton, W. D., Bridle, A. H., 2007, MNRAS, 380, 2

\end{thebibliography}




==> table_1.tex <==
\begin{deluxetable}{llccccc}
\tablecolumns{7}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{{\it HST} Observations \label{HSTTable}}

\tablehead{
\colhead{Instrument} &
\colhead{Filter/Polarizer} &
\colhead{$\lambda_\circ^a$} &
\colhead{FWHM$^b$} &
\colhead{Num Exp$^c$} &
\colhead{Obs Date} &
\colhead{Time (s)$^d$}}

\startdata
WFPC2/PC      & F702W          & 6919  & 1382 & 2 & 12/24/1994 & 280  \\
WFPC2/PC      & F606W          & 5997  & 1502 & 1 & 04/16/1995 & 500  \\
WFPC2/PC      & F791W          & 7881  & 1224 & 2 & 05/19/1996 & 750  \\
WFPC2/PC      & F547M          & 5483  & 484  & 2 & 05/19/1996 & 900  \\
NICMOS/NIC2   & F110W          & 11285 & 3844 & 4 & 05/12/1998 & 448  \\
NICMOS/NIC2   & F160W          & 16030 & 2772 & 4 & 05/12/1998 & 448  \\
NICMOS/NIC2   & F205W          & 20714 & 4314 & 4 & 05/12/1998 & 896  \\
STIS/NUV-MAMA & F25QTZ         & 2354  & 995  & 1 & 02/12/2000 & 1800 \\
STIS/FUV-MAMA & 25MAMA         & 1374  & 318  & 1 & 02/12/2000 & 1705 \\
STIS/FUV-MAMA & F25SRF2        & 1469  & 281  & 1 & 02/12/2000 & 1700 \\
WFPC2/PC      & F702W          & 6919  & 1382 & 9 & 03/30/2002 & 1400 \\
\\
ACS/HRC       & F606W/POL0V    & 5895  & 1588 & 2 & 12/05/2002 & 300  \\
ACS/HRC       & F606W/POL60V   & 5895  & 1588 & 2 & 12/05/2002 & 300  \\
ACS/HRC       & F606W/POL120V  & 5895  & 1588 & 2 & 12/05/2002 & 300  \\
ACS/HRC       & F330W/POL0UV   & 3372  & 410  & 2 & 12/05/2002 & 300  \\
ACS/HRC       & F330W/POL60UV  & 3372  & 410  & 2 & 12/05/2002 & 300  \\
ACS/HRC       & F330W/POL120UV & 3372  & 410  & 2 & 12/05/2002 & 300  \\
WFPC2/PC      & F555W/POLQ$^e$ & 5439  & 1232 & 8 & 03/06/2003 & 6500 \\
WFPC2/PC      & F555W/POLQ$^e$ & 5439  & 1232 & 8 & 04/25/2003 & 6500 \\
WFPC2/PC      & F555W/POLQ$^e$ & 5439  & 1232 & 8 & 06/01/2003 & 6500 \\
\enddata

\tablenotetext{a}{Pivot wavelength of filter in \AA.}

\tablenotetext{b}{Approximate FWHM of filter bandpass in \AA.}

\tablenotetext{c}{Number of images in raw data set (including CR-SPLITs).}

\tablenotetext{d}{Total integration time of all images in seconds.}

\tablenotetext{e}{Due to non-rotatability of the WFPC2 polarizer (POLQ), {\it
HST} was allowed to precess between observations over a $\sim 2$ month time
period, simulating the nominal polarizer angles of $0^\circ$, $60^\circ$, and
$120^\circ$. See text for details.}

\end{deluxetable}


==> table_2.tex <==
\begin{deluxetable}{cccccc}
\tablecolumns{6}
\tablecaption{{\it VLA} Observations \label{VLATable}}

\tablehead{
\colhead{Band} &
\colhead{IF 1/IF 2 (${\rm GHz}$)} &
\colhead{Array Config.} &
\colhead{Max. Baseline (${\rm k\lambda}$)} &
\colhead{Obs. Date} &
\colhead{Time (s)$^a$}}


\startdata
K & 22.4851/22.4351 & B & & 06/23/2002 & \\
\enddata

\tablenotetext{a}{Total integration time in seconds.}

\end{deluxetable}

